STAR-RISs: A Correlated T&R Phase-Shift Model and Practical Phase-Shift Configuration Strategies

A correlated transmission and reflection (T&R) phase-shift model is proposed for passive lossless simultaneously transmitting and reflecting reconfigurable intelligent surfaces (STAR-RISs). A STAR-RIS-aided two-user downlink communication system is investigated for both orthogonal multiple access (OMA) and non-orthogonal multiple access (NOMA). To evaluate the impact of the correlated T&R phase-shift model on the communication performance, three phase-shift configuration strategies are developed, namely the primary-secondary phase-shift configuration (PS-PSC), the diversity preserving phase-shift configuration (DP-PSC), and the T/R-group phase-shift configuration (TR-PSC) strategies. Furthermore, we derive the outage probabilities for the three proposed phase-shift configuration strategies as well as for those of the random phase-shift configuration and the independent phase-shift model, which constitute performance lower and upper bounds, respectively. Then, the diversity order of each strategy is investigated based on the obtained analytical results. It is shown that the proposed DP-PSC strategy achieves full diversity order simultaneously for users located on both sides of the STAR-RIS. Moreover, power scaling laws are derived for the three proposed strategies and for the random phase-shift configuration. Numerical simulations reveal a performance gain if the users on both sides of the STAR-RIS are served by NOMA instead of OMA. Moreover, it is shown that the proposed DP-PSC strategy yields the same diversity order as achieved by STAR-RISs under the independent phase-shift model and a comparable power scaling law with only 4 dB reduction in received power.

==> deleted_materals.tex <==
\textcolor{blue}{
\section{Phase-Shifts Design Through Optimization Algorithms}
To fully exploiting the performance of STAR-RIS under our proposed model, in this section, we jointly consider the optimization of $\Xi'= \{P_R$, $P_T$, $\phi^R_m$ and $\phi^T_m \}$.
To facilitate our optimization algorithm, let us first consider the optimization of a single element $m$, while the phase-shift design of other elements are fixed. For this problem, $\phi^R_m$ and $\phi^T_m$ need to be configured so that to maximum sum rate formulated in \eqref{max} of problem (P0). The maximum is only reached when the total derivative of the sum rate ($R_\Sigma$) is zero, i.e.,
\begin{equation}\label{fraction}
    \delta R_\Sigma = \frac{\partial R_\Sigma}{\partial \phi^R_m} \delta\phi^R_m + \frac{\partial R_\Sigma}{\partial \phi^T_m} \delta\phi^T_m  = 0,
\end{equation}
where $\delta\phi^\chi_m$ is the infinitesimal change of the phase-shift $\phi^\chi_m$ and the partial derivatives ${\partial R_\Sigma}/{\partial \phi^\chi_m}$ are evaluated at the chosen phase-shift value $\phi^R_m$ and $\phi^T_m$. Thus, the partial derivative can be approximated as follows:
\begin{equation}\label{partial}
    \frac{\partial R_\Sigma}{\partial \phi^\chi_m} 
    \approx \frac{2P_\chi|H^\chi|/\sigma^2_\chi}{1+P_\chi|H^\chi|^2/\sigma^2_\chi}\mu^\chi_h\cos\phi^\chi_m,
\end{equation}
where $P_\chi$ and $|H^\chi|$ are the corresponding power and the magnitude of the overall channel within the current optimization iteration.
Moreover, according to the phase-shift constraint \eqref{pha} given in \textbf{Model 1}, we have $\delta\phi^R_m = -\delta\phi^T_m$. 
Thus, by substituting the partial derivative in \eqref{partial} into \eqref{fraction}, the phase-shift values for the $m$th element should be updated according to the following rule:
\begin{equation}\label{rule}
    \frac{2P_R|H^R|/\sigma^2_R}{1+P_R|H^R|^2/\sigma^2_R}\mu^R_h\cos\phi^R_m = \frac{2P_T|H^T|/\sigma^2_T}{1+P_T|H^T|^2/\sigma^2_T}\mu^T_h\cos\phi^T_m
\end{equation}
\begin{algorithm}
	\caption{A1} 
	\begin{algorithmic}[1]
	\State Initiate \{$\phi^R_1,\cdots,\phi^R_M$\} and \{$\phi^T_1,\cdots,\phi^T_M$\} with random values.
		\For {$iteration=1,2,\ldots$}
			\For {$\mathrm{index}=1,2,\ldots,M$}
				\State update $\phi^R_{\mathrm{index}}$ and  $\phi^T_{\mathrm{index}}$ according to \eqref{rule}.
			\EndFor
			\State Optimize and update $P_R$ and $P_T$ using water-filling.
		\EndFor
	\end{algorithmic} 
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%

To maximize the sum rate of user R and user T, we need to jointly consider the optimization of $\Xi = \{P_R$, $P_T$, $\beta^R_m$, $\beta^T_m$, $\phi^R_m$ and $\phi^T_m \}$.
\begin{align}\label{max}
    \text{(P0)}
    \max_{\Xi}& \  \log_2\Big(1+\frac{|H^R|^2P_R}{\sigma_R^2}\Big)+\log_2\Big(1+\frac{|H^T|^2P_T}{\sigma_T^2}\Big)  \\ \label{cons_0}
    \text{s.t.}& \ \  \phi^R_m - \phi^T_m = \frac{\pi}{2} + \nu_m\pi, \ \nu_m=0, 1,\\
    & \ \ (\beta^T_m)^2+(\beta^R_m)^2 = 1,\\
    & \ \ P_T+P_R \leq P_t,
\end{align}
where $P_R$, $P_T$ and $P_t$ are the transmit power for user R, user T and the overall transmit power of BS, respectively, $\sigma^2_\chi$ is the power spectrum density of the Gaussian white noise at user $\chi$.

For simplicity, in the next section,
we first investigate the scenario where the STAR-RIS can be positioned with LoS links to the BS, i.e., $K_g=\infty$. 
Moreover,
we assume that the power ratio between the reflected and transmitted signals at each element is fixed to the same value $\beta^R/\sqrt{1-|\beta^R_m|^2}$, and only investigate the effects of different phase-shift designs.
Using these assumptions, we rewrite the overall channel by separating the amplitude terms and the phase terms as follows:
\begin{equation}\label{sep}
     H^\chi = |g|\beta^\chi \sum_{m=1}^M |h^\chi_m| \exp\{ j(\angle{g_m}+\angle{h^\chi_m+\phi^\chi_m}) \}+h^\chi_d,
\end{equation}
where $\angle{\xi}$ denotes the argument (complex angle) of $\xi$. 
The sum rate optimization problem of the STAR-RIS phase-shifts can be formulated as follows:
\begin{align}\label{max'}
    \text{(P')}
    \max_{\phi^R_m,\phi^T_m}& \  \log_2\Big(1+\frac{|H^R|^2P_R}{\sigma_R^2}\Big)+\log_2\Big(1+\frac{|H^T|^2P_T}{\sigma_T^2}\Big)  \\ \label{cons}
    \text{s.t.}& \ \  \phi^R_m - \phi^T_m = \frac{\pi}{2} + \nu_m\pi, \ \nu_m=0, 1,
\end{align}

\noindent The additional constraint in \eqref{cons} is introduced by the physical nature of the lossless STAR-RIS hardware model. Including this practical constraint introduces new challenges for phase-shift optimization and can significantly affect the overall performance of the STAR-RIS-assisted network.
%
To better understand these effects, we give several practical phase-shift design schemes for the STAR-RIS and analyze their performance. In particular, the outage probabilities, diversity orders and power scaling laws of these schemes are derived and compared with the corresponding upper-bound and lower-bound scenarios.

%%%%%%%%%%%%%%%%%%

\section{The Fast Beam-Splitting Technique}
In this section, we present the proposed FBS technique. This technique enables a STAR-RIS with only one-bit phase-shift control to maintain specular reflection/transmission on one side while achieving beam-splitting on the other side. In addition, the number of beams can be conveniently changed by only adjusting the phase-shift values of a small portion of the elements.

According to \eqref{pha}, for the considered STAR-RIS implementation, the phase difference between the reflection and transmission coefficients can be either $\pi/2$ or $3\pi/2$.
Thus, we assign one control bit to each element to determine this phase difference exclusively.
Without loss of generality, we consider the case of performing beam-splitting on the transmitted signal in the rest of this letter. The FBS technique only requires the STAR-RIS configuring the phase-shift value imposing on the transmitted signal of the $m$th element as follows:
\begin{equation}
    \phi^T_m = 
    \begin{cases}
      (\phi^R_m-\frac{\pi}{2})+ \pi & \text{if $m\Mod p < q$,}\\
      \phi^R_m-\frac{\pi}{2}  & \text{else,}
    \end{cases}       
\end{equation}
where $p$ and $q$ are predetermined integers which control the number and relative strengths of beams produced by the FBS technique. 
For a more detailed inspection, since each element only support one-bit phase control, the phase of the reflection coefficient, i.e., $\phi^R_m$, cannot be configured. For simplicity, we assume that they all share a common value and thus producing a specular reflection (like a mirror). The case where the elements have additional bits for finer adjustment will be discussed in Secion.~\ref{sec_performance}.
In the following, we will analytically demonstrate the effectiveness of this technique and retrieve the relationship between the number of beams and the value $p$.

\begin{figure}[b!]
    \begin{center}
        \includegraphics[scale=0.5]{io_fig/rad5.eps}
        \caption{Radiation pattern for $p=5$.}
        \label{rad5}
    \end{center}
\end{figure}

\begin{figure}[b!]
    \begin{center}
        \includegraphics[scale=0.5]{io_fig/rad8.eps}
        \caption{Radiation pattern for $p=8$.}
        \label{rad8}
    \end{center}
\end{figure}

Consider the wireless channel between a \textit{t-user} and BS through the STAR-RIS, according to the channel model proposed in~\cite{}, the channel gain can be expressed as:
\begin{equation}
    h(\theta^T) \approx \sum_{m=1}^M \frac{T_m \Tilde{U}_m e^{jkd_m}}{d_m}F(\theta^T),
\end{equation}
where $\theta_T$ is the transmission angle,
$\Tilde{U}_m$ is the phase distribution of the incident signal at the STAR-RIS, $d_m = \sqrt{(R\cos\theta^T)^2 + (R\sin\theta-y_m)^2}$ is the distance between the $m$th column and the user, $y_m$ is the $y$-coordinate of the $m$th column, and $F^{\theta^T}$ is the leaning factor.








%%%%%
To enable an independent control of phases of both the reflection and transmission coefficients, we need to allow energy loss at each element. This can be better understand by reformulating $R_m$ and $T_m$ using the surface electric impedance $Z_e$ and magnetic impedance $Z_m$ of the $m$th element~\cite{nature,phy} as follows:
\begin{align}\label{rm}
    R_m& = -\frac{\eta_0}{2Z_e+\eta_0}+\frac{Z_m}{Z_m+2\eta_0},\\ \label{tm}
    T_m& = \frac{2Z_e}{2Z_e+\eta_0} - \frac{Z_m}{Z_m+2\eta_0},
\end{align}
where $\eta_0$ is the free space wave impedance. Using \eqref{rm} and \eqref{tm}, one can verify that a lossless element having $|R_m|^2+|T_m|^2=1$ is equivalent to $Z_e$ and $Z_m$ being purely imaginary. This will exactly lead to the results given in \eqref{amp} and \eqref{pha}. A lossy element, however, has simultaneous positive values of both $\textrm{Re}[Z_e]$ and $\textrm{Re}[Z_m]$~\cite{phy}. According to this result and using \eqref{rm} and \eqref{tm}, we have the following model:
\begin{modelbox}
The modeling for lossless STAR-RISs is as follows:
\begin{equation}
    |R_m|^2+|T_m|^2+2|R_m||T_m||\cos(\phi^T_m-\phi^R_m)| \leq 1,
\end{equation}
and
\begin{equation}
    \phi^R_m, \phi^T_m \in (0,2\pi], \ \forall m=1,2,\cdots, M.
\end{equation}
\end{modelbox}
Comparing \textbf{Model 2} with \textbf{Model 1}, we can clearly see that \textbf{Model 1} has strict correlation between the phases of $R_m$ and $T_m$ while in \textbf{Model 2} these phases are completely free of constraints. According to \eqref{pha}, the phase difference can only be either $\pi/2$ or $3\pi/2$. In other words, the lossless STAR-RIS elements governed by \textbf{Model 1} support only one-bit phase control for the transmitted signals after the phase of the reflected signal is determined. The lossy STAR-RIS elements support independent phase control for both reflected and transmitted signal, however, this comes at a cost of energy loss. In light of this, both the lossless mode and the lossy mode have advantages and disadvantages. In the next section, a initial performance analysis will be given for the purpose of clarifying...
